Local heights on hyperelliptic curves and quadratic Chabauty

Quadratic Chabauty is a $p$-adic method for determining rational points on curves. Local heights are arithmetic invariants used in the quadratic Chabauty method. We present an algorithm to compute these local heights for hyperelliptic curves at odd primes $\ell \neq p$. This algorithm significantly broadens the applicability of quadratic Chabauty to curves which were previously inaccessible due to the presence of non-trivial local heights. We provide numerous examples, including the first quadratic Chabauty computation for a curve having two primes with non-trivial local heights.

==> picard-lefschetz.tex <==
\section{The Picard--Lefschetz isomorphism}

Here's where we should prove the compatibility of Picard--Lefschetz with pushforwards and pullbacks. (The point is to justify why the local heights formula as we use it here agrees with the one from my paper with Netan.)
